Sketch-and-Project Meets Newton Method: Global $\mathcal O(k^{-2})$ Convergence with Low-Rank Updates

In this paper, we propose the first sketch-and-project Newton method with fast $\mathcal O(k^{-2})$ global convergence rate for self-concordant functions. Our method, SGN, can be viewed in three ways: i) as a sketch-and-project algorithm projecting updates of Newton method, ii) as a cubically regularized Newton ethod in sketched subspaces, and iii) as a damped Newton method in sketched subspaces. SGN inherits best of all three worlds: cheap iteration costs of sketch-and-project methods, state-of-the-art $\mathcal O(k^{-2})$ global convergence rate of full-rank Newton-like methods and the algorithm simplicity of damped Newton methods. Finally, we demonstrate its comparable empirical performance to baseline algorithms.

==> ifdefinitions.tex <==
\newif\ifaistats
\newif\ifarxiv
\newif\ifneurips
\newif\ificml
\newif\ifaistatsnot
\newif\ifarxivnot
\newif\ifneuripsnot
\newif\ificmlnot

\newif\ifextension
\newif\ifextensionnot
\extensionfalse
\extensionnottrue
\newif\ifhidden
\newif\ifhiddennot
\hiddenfalse
\hiddennottrue

\aistatsfalse
\arxivfalse
\neuripsfalse
\icmlfalse
\aistatsnottrue
\arxivnottrue
\neuripsnottrue
\icmlnottrue

\ifaistats \aistatsnotfalse \fi
\ifarxiv \arxivnotfalse \fi
\ifneurips \neuripsnotfalse \fi
\ificml \icmlnotfalse \fi
\ifextension \extensionnotfalse \fi
\ifhidden \hiddennotfalse \fi
